Abelian Chern-Simons theory with toral gauge group, modular tensor categories, and group categories

Classical and quantum Chern-Simons with gauge group $\text{U}(1)^N$ were classified by Belov and Moore in \cite{belov_moore}. They studied both ordinary topological quantum field theories as well as spin theories. On the other hand a correspondence is well known between ordinary $(2+1)$-dimensional TQFTs and modular tensor categories. We study group categories and extend them slightly to produce modular tensor categories that correspond to toral Chern-Simons. Group categories have been widely studied in other contexts in the literature \cite{frolich_kerler},\cite{quinn},\cite{joyal_street},\cite{eno},\cite{dgno}. The main result is a proof that the associated projective representation of the mapping class group is isomorphic to the one from toral Chern-Simons. We also remark on an algebraic theorem of Nikulin that is used in this paper.

==> conclusion.tex <==
\chapter{Conclusion}
\label{ch:conclusion}

QUESTION: DO BRAIDED MONOIDAL EQUIVALENT CATEGORIES (THAT ARE THE SAME IN EVERY OTHER WAY)
GIVE ISOMORPHIC TQFTS?

QUESTION: CAN WE USE THIS AS A PLATFORM TO STUDY SPIN-MTCS.
% Moore, Kitaev, Walker
% Jerry Jenquin
% Rowell
% Moore, Segal
